NF-SecRIS: RIS-Assisted Near-Field Physical Layer Security via Secure Location Modulation

The 6G wireless networks impose extremely high requirements on physical layer secure communication. However, the existing solutions usually can only achieve one-dimensional physical layer security (PLS) in the angle dimension, and cannot achieve PLS in the range dimension. In this paper, we propose the NF-SecRIS system, the first range-angle-dependent (2D) PLS near-field communication system based on ultra-large-scale reconfigurable intelligent surface (RIS). We propose the secure location modulation scheme to synthesize the near-field spatial-temporal coding pattern of RIS with extremely low complexity. It ensures that only legitimate user can receive the raw constellations, while potential eavesdroppers at other ranges or angles can only receive the obfuscated constellations. NF-SecRIS operates without requiring synchronization with either transmitter or receiver. We implement a prototype of NF-SecRIS and conduct comprehensive experiments with multiple modulation schemes. The results show that the bit error rate (BER) of legitimate user is below 10^{-4}, while eavesdroppers at other ranges or angles suffer from BER exceeding 40%. It validates the implementation of 2D PLS in near-field communications.

==> 02_Section/02_Preliminary.tex <==

\section{Preliminary}

% 总分结构，以终为始
 In this section, we first compare the near-field spherical wave model with the far-field plane wave model, and then introduce the secrecy capacity of RIS-assisted systems.

\subsection{Near-Field Characteristics}



The electromagnetic field regions are divided into near-field and far-field zones based on propagation distance, each exhibiting distinct wave propagation model. As illustrated in Fig.~\ref{fig_02_near_far_model}, the critical distance separating these regions is $\frac{2L^2}{\lambda}$. Within the near-field zone, electromagnetic wave propagates as spherical wave, whereas in the far-field region the propagation follows a planar wave model. The planar wave characteristics restrict wave dependence solely to angular dimension, without range-dimensional dependence. In contrast, the spherical wave model introduces non-linear phase variations across three-dimensional space, permitting simultaneous beamforming in both range and angular dimensions. This multi-dimensional control capability establishes the foundation for the 2D PLS proposed in this work.

\subsection{Secrecy Capacity}

Generally, secrecy capacity serves as the core metric for evaluating secure communication quality~\cite{1055917,7762075}. It is determined by the difference between the capacity of the main channel and the eavesdropping channel:
% 行间公式：保密容量
\input{05_Equation_tex_module/equ_01_capacity}%
where $C_{s}$ denotes the secrecy capacity. The parameters $P_{0}$, $N_{0}$,  $\bm{h}_{a}$, $\bm{\Theta}$, $\bm{h}_{b}$, $\bm{h}_{e}$ are defined as the signal power, noise power, channel coefficient vector between Alice and RIS, RIS reflection coefficient matrix, channel coefficient vector between Bob and RIS, and channel coefficient vector between Eve and RIS, respectively.

In quasi-static environments, parameters $\bm{h}_{a}$, $\bm{h}_{b}$, and $\bm{h}_{e}$ remain constant, while $\bm{\Theta}$ serves as the key adjustable parameter. When $\bm{\Theta}$ varies over time, it constitutes a spatial-temporal phase pattern $\bm{\Theta}(t)$. Therefore, the essence of RIS-based PLS lies in designing the spatial-temporal phase pattern $\bm{\Theta}(t)$.

% 图片：近远场模型
\input{04_Figure_tex_module/fig_02_far_near}%




==> 02_Section/08_Discussion.tex <==

\section{Discussion and Future Work}

%\subsection{Expand Effective Range of Secure Communications}

NF-SecRIS represents the first 2D secure communication system based on an ultra-large-scale RIS, achieving an effective secure communication range of 2 meters in its current implementation. Further extension of this range is essential. The primary limitation stems from discrepancies between the actual near-field beam behavior and the expected ideal performance. To enhance the precision of near-field beam control and extend the effective coverage, improvements can be made in the following three aspects.

First, it is necessary to develop a fast and accurate near-field analysis model. Without loss of generality, a simplified near-field model is initially employed to rapidly validate the effectiveness of NF-SecRIS with low computational complexity.
The simplified model deliberately omits certain practical electromagnetic parameters such as the radiation pattern of the horn antenna, the directivity of RIS elements, the actual angles of incidence and reflection per unit, and phase errors in RIS elements. However, full-wave electromagnetic simulation software (e.g., CST, HFSS) is unsuitable for modeling ultra-large-scale RIS due to prohibitive computational resource and time requirements, which contradicts the low-complexity objective of NF-SecRIS. Therefore, future work should focus on creating fast and accurate near-field analysis models that incorporate these practical electromagnetic parameters. Such models would enable the acquisition of accurate field distributions, support the optimization of phase configurations, and ultimately contribute to extending the effective near-field range. This approach holds significant research value and could also be pursued as an independent research topic.

Second, designing RIS elements with wider beamwidth can help mitigate the impact of varying angles of incidence and reflection. In near-field scenarios, significant differences exist in the incident angles across the array, similarly for the reflection angles. For instance, in this study, the incident angle is $0^{\circ}$ for the central element, but reaches $44.2^{\circ}$ for edge elements, resulting in considerable variation in insertion loss and reflection phase. Employing wide-beam elements can reduce angular sensitivity, improve unit-to-unit performance consistency, facilitate effective aperture expansion, and thereby contribute to extending the near-field range.

Third, further increasing the aperture size of the RIS array offers the most direct approach to extending the effective near-field range. To improve the efficiency of edge elements, this strategy should be implemented in conjunction with the previous two solutions.

Our current work has successfully demonstrated the feasibility and effectiveness of the SLM scheme in NF-SecRIS. Future work will focus on implementing the above strategies to further extend the secure communication range of the system.

%%%%%%%%
% 引用文中近场分析公式
   

%\subsection{Noise Time-Slot Processing}

%In the current scheme, the legitimate user Bob directly demodulates the signals reflected by the RIS without specifically filtering out the noise slots. The key advantage of this approach lies in its simplicity, as it requires no modifications to the communication protocols or signal processing procedures. However, an area for future enhancement is that the noise slots still introduce slight interferences to Bob, even though such interferences have been suppressed as much as possible. Therefore, in future work, Bob’s signal processing procedure could be modified to explicitly filter out noise slots, thereby minimizing the interferences caused by the RIS. This enhancement will increase system design complexity, so we should make a careful trade-off between performance and complexity.


%\subsection{RIS Near-Field Transmitter}

%In NF-SecRIS, the RIS functions as a reflective surface for modulated signals, while the transmitter employs a directional antenna to transmit the modulated signals toward the RIS. However, there remains a risk of information leakage to eavesdroppers through direct line-of-sight propagation from Alice to Eves. To completely eliminate the information leakage, NF-SecRIS can be further upgraded into a near-field transmitter. Unlike the current design, the RIS would no longer serve as a reflective surface but would instead act as a transmitter capable of generating baseband signals. In this configuration, the feed antenna would only supply an unmodulated carrier, while the FPGA in the RIS would be responsible for generating both baseband and interference signals. As a result, any electromagnetic leakage from the feed antenna toward eavesdroppers would carry no information. We leave such improvement for our future exploration.


%%%%%%%%
% 增加讨论项：扩展到3d保密，保密球。本次使用的ris在水平面口径远大于垂直面口径，着重关注水平面保密性能，未来可扩展垂直面口径，实现3d保密球。增加3d立体采样点。


==> 02_Section/10_Acknowledgement.tex <==

\section*{Acknowledgments}


\textcolor{blue}{XXX XXX XXX XXX XXX} 

==> 02_Section/12_Biography.tex <==
 
\vspace{11pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{03_Figure_file/fig_01}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}



\vfill

==> 04_Figure_tex_module/fig_02_far_near.tex <==
% 图片：近远场传播模型
\begin{figure}[!t]
\centering
% 子图a
\subfloat[Near-field model]{\includegraphics[height=110pt]{03_Figure_file/fig_02a_nearfieldmodel.pdf}%
\label{fig_02a_近场模型}}
\hfil
% 子图b
\subfloat[Far-field model]{\includegraphics[height=110pt]{03_Figure_file/fig_02b_farfieldmodel.pdf}%
\label{fig_02b_远场模型}}
% 总标题
\caption{Electromagnetic wave propagation model. (a) Near-field spherical wavefront model. (b) Far-field planar wavefront model.}
% 总标签
\label{fig_02_near_far_model}
\end{figure}

==> 05_Equation_tex_module/equ_01_capacity.tex <==
%
%
%
%
% 行间公式：保密容量
\begin{align}
C_{s} 
&=\log_{2}(1+\left|\bm{h}_{b}^{H}\bm{\Theta}\bm{h}_a                                  \right|^2\frac{P_{0}}{N_{0}})
-\log_{2}(1+\left|\bm{h}_{e}^{H}\bm{\Theta}\bm{h}_a                                  \right|^2\frac{P_{0}}{N_{0}}),
\label{eq_01_capacity}
\end{align}%
%
%
% \begin{align}
% C_{s} 
% &= C_{m} - C_{w} \notag\\
% &=\log_{2}(1+\left|\bm{h}_{b}^{H}\bm{\Theta}\bm{h}_a                                  \right|^2\frac{P_{0}}{N_{0}}) \notag\\
% & \quad\, -\log_{2}(1+\left|\bm{h}_{e}^{H}\bm{\Theta}\bm{h}_a                                  \right|^2\frac{P_{0}}{N_{0}}),
% \label{eq_01_capacity}
% \end{align}

==> 05_Equation_tex_module/equ_15_EVM_SNR.tex <==
%
%
%
%
%
%
%
%
% 公式：EVM与SNR关系
\begin{align}
    \text{EVM} \approx \frac{1}{\sqrt{\text{SNR}}},
\end{align}

==> 05_Equation_tex_module/equ_19_gama_interleaving.tex <==
%
%
%
%
%
%
%
%
% 公式：联合编码序列
\begin{align}
    \bm{\Gamma}^{\text{inter}}= \;( \;
    & \bm{\Gamma}_{1}^{\text{focus}}, \bm{\Gamma}_{2}^{\text{focus}}, ..., \bm{\Gamma}_{\frac{K^{\text{focus}}}{K^{\text{null}}}}^{\text{focus}}, \bm{\Gamma}_{1}^{\text{null}}, \notag\\
    & \bm{\Gamma}_{\frac{K^{\text{focus}}}{K^{\text{null}}}+1}^{\text{focus}}, ..., \bm{\Gamma}_{\frac{2K^{\text{focus}}}{K^{\text{null}}}}^{\text{focus}}, \bm{\Gamma}_{2}^{\text{null}}, \notag\\
    & \bm{\Gamma}_{\frac{2K^{\text{focus}}}{K^{\text{null}}}+1}^{\text{focus}}, ..., \bm{\Gamma}_{K^{\text{focus}}}^{\text{focus}}, \bm{\Gamma}_{K^{\text{null}}}^{\text{null}}
    \;) ,
\end{align}
